Thermal effective actions from conformal boundary conditions in gravity

Recent work has studied the thermodynamics of gravity subjected to conformal boundary conditions, where the trace of the extrinsic curvature $K$ and the conformal class of metrics are kept fixed. The case $K < 0$ seems tied to solutions with cosmic horizons. To study this situation further, we analyze Einstein-Maxwell theory, where we find solutions with cosmic horizons corresponding to patches inside the inner horizon of the Reissner-Nordstr\"om black hole. We find that these solutions are $\it{necessary}$ for consistency with the thermal effective action in the putative boundary dual at $O(1)$ chemical potential. Furthermore, we introduce a (positive or negative) cosmological constant and find more cases where solutions with cosmic horizons dominate the ensemble. Transitions between solutions with cosmic horizons and solutions with black hole horizons are mediated by "extremal" solutions that correspond to patches of (A)dS$_2 \times \Sigma^{d-1}$, for which we discuss an effective JT gravity description with dimensionally reduced conformal boundary conditions. Finally, we introduce rotation in some simple cases and find that the bulk theory reproduces the universal velocity-dependent modification of the free energy predicted by the thermal effective action.

==> figs/AdSUncharged/texCode/penroseDiagrams/penroseAdSHyper.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.35]
%% AdS Hyperbolic BH
\draw[draw=none,pattern = crosshatch,pattern color=penroseblue] (1,3) .. controls (0.45,2.25) and (0.45,1.75) .. (1,1) to (0,2) -- cycle;
\draw[draw=none,pattern = crosshatch,pattern color=penrosered] (1,1) .. controls (0.45,0.25) and (0.45,-0.25) .. (1,-1) to (0,0) -- cycle;

% conf boundaries
\draw[-] (-1,-1) to (-1,1);
\draw[-] (1,-1) to (1,1);
% outer horizons
\draw[-,penrosered!80!black,dashed,very thick] (-1,1) to (0,0) to (-1,-1);
\draw[-,penrosered!80!black,dashed,very thick] (1,1) to (0,0) to (1,-1);
% inner horizons
\draw[-,penroseblue!80!black,dashed,very thick] (-1,1) to (1,3);
\draw[-,penroseblue!80!black,dashed,very thick] (1,1) to (-1,3);
\draw[-,penroseblue!80!black,dashed,very thick] (-1,-1) to (1,-3);
\draw[-,penroseblue!80!black,dashed,very thick] (1,-1) to (-1,-3);
% singularities
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (-1,1) to (-1,3);
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (1,3) to (1,1);
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (-1,-3) to (-1,-1);
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (1,-1) to (1,-3);
% labels
\node[penrosered!80!black] at (0.35,0.7) {\large$r_+$};
\node[penrosered!80!black] at (0.35,-0.7) {\large$r_+$};

\node[penroseblue!80!black] at (0.35,2+0.7) {\large$r_-$};
\node[penroseblue!80!black] at (0.35,2-0.7) {\large$r_-$};

\node[rotate=90] at (0,3.25) {\LARGE$\cdots$};
\node[rotate=90] at (0,-3.25) {\LARGE$\cdots$};

\draw[-] (1,3) .. controls (0.45,2.25) and (0.45,1.75) .. (1,1);
\draw[-] (1,1) .. controls (0.45,0.25) and (0.45,-0.25) .. (1,-1);

\node at (0.775,2) {\large$r_c$};
\node at (0.775,0) {\large$r_c$};

\node at (-1.75,0) {};
\node at (1.75,0) {};
\end{tikzpicture}

\caption{The Penrose diagram for the hyperbolic AdS black hole with negative mass $\m < 0$. We can construct both black hole patches (in red) and  cosmic patches (in blue).}
\label{figs:penroseAdSHyper}
\end{figure}

==> figs/AdSUncharged/texCode/phasePlots/phasesAdSPlanar.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\node[white] at (4.5,0) {$\bullet$};
\node at (0,0){\includegraphics[scale=0.6]{figs/AdSUncharged/planar/phasesAdSPlanar.png}};
\node at (0.46,-2.125) {\footnotesize{\textcolor{white}{\textbf{No solutions}}}};
\node at (0.46,1.2) {\footnotesize\shortstack{\textcolor{white}{\textbf{Black hole}}\\\textcolor{white}{\textbf{(stable)}}}};
\end{tikzpicture}
\caption{This is the analytic phase diagram (in any dimension) for the $\L < 0$ case with a toroidally compactified spatial boundary. There is a first-order phase transition between the black hole brane and the AdS soliton at $\tilde{\b}/\tilde{L}_{\text{min}} = 1$, and there are no solutions below $K\ell = d$.}
\label{figs:phasesAdSPlanar}
\end{figure}

==> figs/dSUncharged/texCode/penroseDiagram/penrosedSHyperPlanar.tex <==
\begin{figure}
\centering
\hspace{80mm} \begin{tikzpicture}[scale=1.35]
\draw[draw=none,pattern = crosshatch,pattern color=penroseblue] (1,1) .. controls (0.45,0.25) and (0.45,-0.25) .. (1,-1) to (0,0) -- cycle;

% conf boundaries
\draw[-] (-1,-1) to (1,-1);
\draw[-] (-1,1) to (1,1);
% outer horizons
\draw[-,penroseblue!80!black,dashed,very thick] (-1,1) to (0,0) to (-1,-1);
\draw[-,penroseblue!80!black,dashed,very thick] (1,1) to (0,0) to (1,-1);
% singularities
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (-1,-1) to (-1,1);
\draw[-,decorate,decoration={zigzag,amplitude=0.5mm,segment length=2.5mm}] (1,-1) to (1,1);
% labels
\node[penroseblue!80!black] at (0.35,0.7) {\large$r_h$};
\node[penroseblue!80!black] at (0.35,-0.7) {\large$r_h$};


\draw[-] (1,1) .. controls (0.45,0.25) and (0.45,-0.25) .. (1,-1);

\node at (0.775,0) {\large$r_c$};

\node at (0,-1.5) {};
\node at (0,1.5) {};
\end{tikzpicture}

\caption{The Penrose diagram for the planar, hyperbolic, and negative-mass $\m < 0$ dS black holes. The only solutions consistent with conformal boundary conditions are cosmic patches, shown in blue.}
\label{figs:penrosedSHyperPlanar}
\end{figure}

==> figs/dSUncharged/texCode/phasePlots/phasesdSHyper.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\node at (0,0){\includegraphics[scale=0.75]{figs/dSUncharged/hyperbolic/phasesdSHyper.png}};
\node at (8.125,0) {};

\node at (4.925,2.435-0.65) {\footnotesize{\textcolor{white}{\textbf{No solution}}}};
\node at (-1.8,0.525) {\footnotesize{\textcolor{white}{\textbf{Cosmic (stable)}}}};
\end{tikzpicture}
\caption{This is the phase diagram for $\L > 0$, $d=3$ with hyperbolic slices $k=-1$. The larger of the two cosmic solutions in the $(0,2)$ region from Figure \ref{fig:solutionsdSHyper} is the stable one. Due to the lack of a thermal gas solution, we have no candidate solution for part of the phase diagram.}
\label{fig:phasesdSHyper}
\end{figure}

==> figs/flatCharged/texCode/phasePlots/phasesFlatHyperCharged.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\node[white] at (4.5,0) {$\bullet$};
\node at (0,0){\includegraphics[scale=0.6]{figs/flatCharged/hyperbolic/phasesFlatHyperCharged.png}};
\node at (1.25,1.4) {\footnotesize{\textcolor{white}{\textbf{No solution}}}};
\node at (0.7,-2.1375+0.37) {\footnotesize{\textcolor{white}{\textbf{Cosmic (unstable)}}}};
\node at (-1.375,-1+0.65) {\footnotesize\shortstack{\textcolor{white}{\textbf{Cosmic}}\\\textcolor{white}{\textbf{(stable)}}}};
\end{tikzpicture}
\caption{The phase diagram for the hyperbolic horizon topology in $d = 3$. This also doubles as the stability plot; the larger cosmic solution in the $K>0$ region is dominant and stable, while the cosmic solution in the $K<0$ region is dominant and unstable.}
\label{figs:phasesFlatHyperCharged}
\end{figure}

==> figs/flatCharged/texCode/solutionSpaces/criticalPointsflatSphereCharged.tex <==
\begin{figure}
\centering
\subfloat[Left critical point ($\tilde{\beta} = \tilde{\beta}_{\text{L}}$)]{
\includegraphics[scale=0.75]{figs/flatCharged/sphere/critLeft.pdf}
}\quad\quad
\subfloat[Right critical point ($\tilde{\beta} = \tilde{\beta}_{\text{R}}$)]{
\includegraphics[scale=0.75]{figs/flatCharged/sphere/critRight.pdf}
}
\caption{Plots of $\tilde{\Phi}K$ as a function of $z$ at $d = 3$ for (a) the left critical point $\tilde{\beta} = \tilde{\beta}_{\text{L}}$ and (b) the right critical point $\tilde{\beta} = \tilde{\beta}_{\text{R}}$, which we respectively find to be (approximately) 6.7841 and 6.8927. Red denotes the \textcolor{red}{black-hole branch ($z < 1$)}, and blue denotes the \textcolor{blue}{cosmic branch ($z > 1$)}. The values of $\tilde{\beta}$ in each case are finely tuned such that, for increasing $\tilde{\Phi}K$, the $(1,0)$ region transitions directly to either the $(2,1)$ region or the $(3,0)$ region.}
\label{figs:plotsPhiKCriticalPoints}
\end{figure}
